Cramer-Castillon on a Triangle's Incircle and Excircles

The Cramer-Castillon problem (CCP) consists in finding one or more polygons inscribed in a circle such that their sides pass cyclically through a list of $N$ points. We study this problem where the points are the vertices of a triangle and the circle is either the incircle or excircles.

==> 001_scenario.tex <==
\begin{itemize}
    \item shared X6, X15, X16, and $\Omega_1,\Omega_2$, brocard axis, and Brocard inellipse -- meaning, the two triangles are in the same harmonic family (Brocard porism)
  \item locus of X6 is an ellipse. what are its axes?
  \item cot(w1) = cot(w2)
  \item what is the locus of the brocard points?
 \item what are the dynamics of the Brocard inellipse
\item we have two methods to find the solution (Carnot+Mobius, Dominique Synthetic Method, and an iterative dynamical map
\item are the 6 sides of the 2 triangles tangent to the same conic? they each will define one conic which w the outer one defines a poncelet family.
\end{itemize}

==> 240_app_moses.tex <==
In this appendix we provide expressions for the solutions of the CCP-on-the-incenter using barycentrics. Here $a,b,c$ denote the sidelengths.

\subsection*{A-vertex of $T_1$} $[-(a+b-c) (a-b+c) (\phi-2)^2,(a-b-c) (a+b-c) (\phi-1)^2,(a-b-c) (a-b+c)]$.

\subsection*{A-vertex of $T_2$} $[-(a+b-c) (a-b+c) (\phi-2)^2,(a-b-c) (a+b-c),(a-b-c) (a-b+c) (\phi-1)^2]$.

\subsection*{First Brocard point of either solution}
$[-(a+b-c) (a-b+c) (a^2-2 a b+b^2-a c-b c),-(a-b-c) (a+b-c) (a b-b^2+a c+2 b c-c^2),(a-b-c) (a-b+c) (a^2-a b-2 a c-b c+c^2)]$.

\subsection*{Second Brocard point of either solution} $
[-(a+b-c) (a-b+c) (a^2-a b-2 a c-b c+c^2),(a-b-c) (a+b-c) (a^2-2 a b+b^2-a c-b c),-(a-b-c) (a-b+c) (a b-b^2+a c+2 b c-c^2)]$

\subsection*{Shared triangle centers}

The following pairs $[i,k]$ of $X_i$ of either solution and $X_j$ of the reference are shared: $[3,1]$, $[6,7]$, $[15,3638]$,  $[16,3639]$,  $[32,10481]$,  $[182,5542]$,  $[187,1323]$,  $[371,482]$,  $[372,481]$,  $[511,516]$,  $[512,514]$,  $[575,43180]$,  $[576,30424]$,  $[1151,176]$,  $[1152,175]$,  $[1350,390]$,  $[1351,4312]$,  $[1384,21314]$,  $[2076,14189]$,  $[3053,279]$,  $[3098,30331]$,  $[3311,1373]$,  $[3312,1374]$,  $[3592,21169]$,  $[5017,42309]$,  $[5023,3160]$,  $[5085,11038]$,  $[5585,31721]$,  $[5611,10652]$,  $[5615,10651]$,  $[6200,31538]$,  $[6221,1371]$,  $[6396,31539]$,  $[6398,1372]$,  $[6409,17805]$,  $[6410,17802]$,  $[6419,21171]$,  $[6425,31601]$,  $[6426,31602]$,  $[6431,21170]$,  $[6437,17804]$,  $[6438,17801]$,  $[6449,17806]$,  $[6450,17803]$,  $[11824,31567]$,  $[11825,31568]$,  $[12305,30333]$,  $[12306,30334]$,  $[14810,43179]$,  $[15815,5543]$,  $[21309,20121]$,  $[31884,8236]$,  $[43118,30342]$,  $[43119,30341]$,  $[43120,31570]$,  $[43121,31569]$.

\subsection{Dominique overflow}

Below we provide barycentric coordinates for a few notable points shared by the Cramer-Castillon triangles in the incircle of a triangle $T=ABC$ with respect to the latter:

\subsection{First Brocard points} its barycentrics $[w_{11},w_{12},w_{13}$ are given by:

\begin{align*}
w_{11} &= \frac{1}{2w}(a^2 - 2ab + b^2 - a c - b c)(a + b - c)(a - b + c)\\
w_{12} &=  \frac{1}{2w}(ab - b^2 + ac + 2b c - c^2)(a + b - c)(a - b - c)\\
w_{13} &= 1 - w_{11}  - w_{12}
\end{align*}
where: $w = a^3b - 2a^2b^2 + ab^3 + a^3c - a^2bc - ab^2c + b^3c - 2a^2c^2 - abc^2 - 2b^2c^2 + ac^3 + bc^3$.

\subsection{2nd Brocard point} its barycentrics $[w_{21},w_{22},w_{23}]$ are given by:

\begin{align*}
w_{21} &= \frac{1}{2w}(a^2 - ab - 2ac - bc + c^2)(a + b - c)(a - b + c)\\
w_{22} &=  -\frac{1}{2w}(a^2 - 2ab + b^2 - ab - bc)(a + b - c)(a - b - c)\\
w_{23} &= 1 - w_{21}  - w_{22}
\end{align*}

\subsection{Symmedian point} Its barycentrics $[z_1,z_2,z_3]$ are given by:

\begin{align*}
z_{1} &= \frac{-(a + b - c)(a - b + c)}{(a^2 - 2ab + b^2 - 2ac - 2bc + c^2)}\\
z_{2} &=  \frac{(a + b - c)(a - b - c)}{(a^2 - 2ab + b^2 - 2ac - 2bc + c^2)}\\
z_{3} &= 1 - z_{1}  - z_{2}
\end{align*}

\subsection{Corresponding triangle centers}

==> 998_refs_dom.tex <==
@article{BSMF_1891__19__133_0,
     author = {Lemoine, \'Emile},
     title = {Sur une transformation relative \`a la g\'eom\'etrie du triangle},
     journal = {Bulletin de la Soci\'et\'e Math\'ematique de France},
     pages = {133--135},
     publisher = {Soci\'et\'e math\'ematique de France},
     volume = {19},
     year = {1891},
     doi = {10.24033/bsmf.437},
     language = {fr},
     url = {http://www.numdam.org/articles/10.24033/bsmf.437/}
}

==> 999_peter_notes.tex <==


\[
T_{1,exc} =
\begingroup % keep the change local
\setlength\arraycolsep{10pt}
\begin{bmatrix}
-8 (s-c) (s-b) k_1 &  (s-b) s k_2 &  (s-c)  s  k_3 \\
-8 (s-c) (s-b) k_1 & (s-b) s k_2 &  (s-c)  s  k_4 \\
-8 (s-c)  (s-b) k_5 &  (s-b) s k_2 &  (s-c)  s  k_4
\end{bmatrix}\endgroup
\]
where:

\begin{align*}
k_1=&(\sqrt{5} a + b - c)^2 \\
k_2=&(5 a + b - c +2\sqrt{5}  (s-c))^2 \\
k_3=&(-5 a + b - c + 2\sqrt{5} (s-b))^2\\
k_4=&(5 a + 3 b - 3 c + \sqrt{5} (3 a + b - c))^2\\ 
k_5=&(5 a + 2 b - 2 c  +\sqrt{5} (2 a + b - c))^2
\end{align*}


==> 999_refcheck.tex <==
\usepackage{refcheck}
% make refcheck work w cref
% https://tex.stackexchange.com/questions/87610/making-refcheck-work-with-cleveref
\makeatletter
\newcommand{\refcheckize}[1]{%
  \expandafter\let\csname @@\string#1\endcsname#1%
  \expandafter\DeclareRobustCommand\csname relax\string#1\endcsname[1]{%
    \csname @@\string#1\endcsname{##1}\@for\@temp:=##1\do{\wrtusdrf{\@temp}\wrtusdrf{{\@temp}}}}%
  \expandafter\let\expandafter#1\csname relax\string#1\endcsname
}
\newcommand{\refcheckizetwo}[1]{%
  \expandafter\let\csname @@\string#1\endcsname#1%
  \expandafter\DeclareRobustCommand\csname relax\string#1\endcsname[2]{%
    \csname @@\string#1\endcsname{##1}{##2}\wrtusdrf{##1}\wrtusdrf{{##1}}\wrtusdrf{##2}\wrtusdrf{{##2}}}%
  \expandafter\let\expandafter#1\csname relax\string#1\endcsname
}
\makeatother

\refcheckize{\cref}
\refcheckize{\Cref}
\refcheckizetwo{\crefrange}
\refcheckizetwo{\Crefrange}
